Bitcoin-Enhanced Proof-of-Stake Security: Possibilities and Impossibilities

Bitcoin is the most secure blockchain in the world, supported by the immense hash power of its Proof-of-Work miners. Proof-of-Stake chains are energy-efficient, have fast finality but face several security issues: susceptibility to non-slashable long-range safety attacks, low liveness resilience and difficulty to bootstrap from low token valuation. We show that these security issues are inherent in any PoS chain without an external trusted source, and propose a new protocol, Babylon, where an off-the-shelf PoS protocol checkpoints onto Bitcoin to resolve these issues. An impossibility result justifies the optimality of Babylon. A use case of Babylon is to reduce the stake withdrawal delay: our experimental results show that this delay can be reduced from weeks in existing PoS chains to less than 5 hours using Babylon, at a transaction cost of less than 10K USD per annum for posting the checkpoints onto Bitcoin.

==> accountable_liveness.tex <==
\subsection{Liveness Violation is not Accountable}
\label{sec:accountable-liveness}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/inactivity_leak.jpg}
    \caption{Inactivity leak attack. At the top is adversary's private attack chain. At the bottom is the public canonical chain built by the honest validators.
    Due to inactivity leak, honest and adversarial validators lose their stake on the attack and canonical chains respectively. A late-coming client cannot differentiate the canonical and attack chains.}
    \vspace{-0.2in}
    \label{fig:inactivity-leak}
\end{figure}

Without additional trust assumptions, clients cannot identify any validator to have irrefutably violated the protocol in the event of a liveness violation, even with a static set of validators and a synchronous network.
To illustrate the intuition behind this claim, we analyze \emph{inactivity leak}~\cite{inactivity_leak} proposed as financial punishment for inactive PoS Ethereum validators.
We show that when the adversary is sufficiently strong, inactivity leak can result in a gradual slashing of the honest validators' stake in the view of a \emph{late-coming} client with non-negligible probability.

Consider the setup on Figure~\ref{fig:inactivity-leak}, where half of the validators are adversarial and build a private attack chain.
They do not communicate with the honest validators while constructing the private chain, thus, lose their stake on the canonical chain due to inactivity leak.
However, as the honest validators are not privy to the adversary's actions, they also cannot vote for the blocks, or be part of the protocol execution on the attack chain.
As a result, they also lose their stake on the attack chain due to inactivity leak.
Finally, the adversary publishes the attack chain, which is subsequently seen by a late-coming client.

Upon seeing the two chains, the late-coming client has two possible actions: 
It can reject both of the chains, in which case liveness is violated, and no adversarial validator is slashed.
Alternatively, it can accept and output one of the chains.
As the late-coming client could not have observed the attack in progress, it cannot irrefutably identify which of the chains is the attack chain.
Thus, with non-negligible probability, the late-coming client outputs the attack chain, in which case the stake of the honest validators would be slashed in the client's view.

The following theorem generalizes the observation above to all \pos protocols:
\begin{theorem}
\label{thm:accountable-liveness}
Without additional trust assumptions, no permissioned or \pos protocol provides both $\fA$-$\Tconfirm$-accountable-liveness and $\fS$-safety for any $\fA,\fS > 0$ and $\Tconfirm<\infty$ in a $\Delta$-synchronous network.
\end{theorem}

\begin{proof}[Proof of Theorem~\ref{thm:accountable-liveness}]
Towards contradiction, suppose there exists a \pos protocol $\PI$ with a static set of $n$ validators that provides $\fA$-$\Tconfirm$-accountable-liveness and $\fS$-safety for some integers $\fA,\fS>0$ and $\Tconfirm<\infty$.
Let $\fL$ denote the liveness resilience of $\PI$.
By Theorem~\ref{thm:sync-tradeoff}, $\fL < n - \fS$, \ie, $\fL < n-1$ as $\fS > 0$.
Let $m$ denote the maximum integer less than $n-\fL$ that divides $n$.
There exists such an integer since $n-\fL>1$.
Let $P_i$, $i \in [n/m]$, denote sets of size $m$ that partition the $n$ validators into $n/m$ disjoint, equally sized groups.
Consider the following worlds indexed by $i \in [n/m]$, where $\Env$ inputs transaction $\tx_i$ to the validators in $P_i$ at slot $0$.
Here $\tx_i \neq \tx_j$ for $i \neq j$.

\textbf{World $i$:}
Validators in $P_i$ are honest.
Validators in $P_j$, $j \neq i, j \in [n/m]$, are adversarial, and in their heads, simulate the execution of $m$ honest validators that do not receive any messages from those in the other sets.
There is a single client $\node$.
At slot $\Tconfirm$, $\node$ queries the validators and receives responses from all of the validators, upon which, it outputs the chain $\poschain^{\node}_{\Tconfirm}$.
As $|P_i| < n-\fL$ and the validators in $P_i$ do not receive any message from the other validators, it holds that $\tx_i \notin \poschain^{\node}_{\Tconfirm}$.
Similarly, as the validators in each of the sets $P_j$, $j \neq i, j \in [n/m]$ simulate the execution of honest validators that do not receive any messages from those in the other sets, for all $j \neq i, j \in [n/m]$, it also holds that $\tx_j \notin \poschain^{\node}_{\Tconfirm}$.
Thus, there is a liveness violation, and $\node$ asks the validators for their transcripts.
As $\fA>0$, by invoking the forensic protocol with the transcripts received, it identifies a non-empty subset $S_i$ of the adversarial validators.

By definition, $S_i \subseteq \bigcup_{j \in [n/m], j \neq i} P_j$.
However, as the worlds $i$, $i \in [n/m]$ are indistinguishable for $\node$, there exists a world $i^*$, $i^* \in [n/m]$, such that a validator in $P_{i^*}$ is identified by the forensic protocol in world $i^*$.
This is a contradiction.
\end{proof}

Since $f$-\slr implies $f$-\alr for any \pos protocol, Theorem~\ref{thm:accountable-liveness} implies that no \pos protocols can have a positive \emph{\slr}.
\begin{corollary}
\label{cor:pos-non-slashable-liveness}
Without additional trust assumptions, no \pos protocol provides both $\fS$-safety and $\fL$-$\Tconfirm$-slahable-liveness for any $\fS,\fL>0$ and $\Tconfirm<\infty$ under a $\Delta$-synchronous network.
\end{corollary}
